Fine-tuned LLMs Know More, Hallucinate Less with Few-Shot Sequence-to-Sequence Semantic Parsing over Wikidata

While large language models (LLMs) can answer many questions correctly, they can also hallucinate and give wrong answers. Wikidata, with its over 12 billion facts, can be used to ground LLMs to improve their factuality. This paper presents WikiWebQuestions, a high-quality question answering benchmark for Wikidata. Ported over from WebQuestions for Freebase, it consists of real-world data with SPARQL annotation. This paper presents a few-shot sequence-to-sequence semantic parser for Wikidata. We modify SPARQL to use the unique domain and property names instead of their IDs. We train the parser to use either the results from an entity linker or mentions in the query. We fine-tune LLaMA by adding the few-shot training data to that used to fine-tune Alpaca. Our experimental results demonstrate the effectiveness of this methodology, establishing a strong baseline of 76% and 65% answer accuracy in the dev and test sets of WikiWebQuestions, respectively. By pairing our semantic parser with GPT-3, we combine verifiable results with qualified GPT-3 guesses to provide useful answers to 96% of the questions in dev. We also show that our method outperforms the state-of-the-art for the QALD-7 Wikidata dataset by 3.6% in F1 score.

==> background.tex <==
\section{Background of Wikidata}
\TODO{Compress this for space reason.}
A knowledge base (KB) is a structured database consisting of a set of entities and relationships between them.
KBs store facts in the form of subject-relation-object triples. 
In each triple, the subject is an entity while the object could be either an entity or a literal, such as a date or a number.
Large knowledge bases, such as Freebase \citep{freebase}, DBPedia \citep{dbpedia}, and Wikidata \citep{fb2wd},
store an enormous amount of human knowledge in various domains. They provide structured web information for various downstream tasks including web search. 

%Freebase was launched in 2007 by Metaweb and later acquired by Google in 2010. It served as the open core of the Google Knowledge Graph. Wikidata was a public knowledge base that started in 2012; it grew so quickly that Freebase was shut down and integrated into Wikidata by 2014.  

As of May 2023, Wikidata has over 10,000 properties, 100 million entities, and 12 billion facts, making it the biggest public knowledge base.  
Note that only 3,000 of the properties are needed for answering user questions; the rest are used to link data in Wikidata with external library catalogs and database IDs. 

Figure~\ref{fig:wikidata-entry} shows an example Wikidata page for entity ``Joe Biden''. 
In Wikidata, entities and properties are given unique identifiers, QIDs and PIDs, respectively, and a default natural language label. It also contains a description and aliases providing alternative ways to describe the entity or property. 
Label, description, and aliases are all multilingual, meaning that they can be displayed to users or entered by users in all languages supported. 

Facts are stored as statements in Wikidata.
For example, the fact that Joe Biden is the president of the United States can be represented as a statement triple 
(Q6279, P39, Q11696), where P39 is the PID for property {\em position held}, Q6279 and Q11696 are QIDs for Joe Biden and the president of the United States, respectively. 
Each statement can be qualified with additional conditions. For example, ``Joe Biden is the president of the US'' is qualified by the predicate (P580, 20 Jan 2021), meaning that the {\em start time} (P580) of Joe Biden's presidency is 20 Jan 2021.

\begin{figure}
    \centering
    \includegraphics[width=0.46\textwidth]{figures/wikidata-entry.pdf}
    \caption{An example Wikidata page: Joe Biden.} 
    \label{fig:wikidata-entry}
\end{figure}

Unlike Freebase, Wikidata does not have a fixed set of domains with their available properties as schema. 
Instead, any entity can be used as a subject or an object with any property to form a triple. 
However, each entity has a property {\em instance of} (P31) that lists the {\em domain entities} the entity belongs to.
For example, ``Joe Biden'' is an instance of ``human'' as shown in Figure~\ref{fig:wikidata-entry}.
Each domain entity has a {\em subclass of} (P279) property that lists its higher-level domain entities, forming a hierarchical type system.
For example, ``human'' domain is a subclass of ``mammal'', which is a subclass of ``vertebrate'', which is a subclass of ``animal''. All domains are a subclass of the ``entity'' domain. 


==> domain-types.tex <==
\section{Property-Based Knowledge Graphs}

%As it is infeasible to collect enough natural human questions to adequately cover possible questions on  Wikidata, we augment the training data set with synthesized data. It is challenging to generate good synthesis data for Wikidata. 
Wikidata is the largest public knowledge base with over 12 billion facts represented by subject-predicate-object triples using 10,000 properties and 100 million entities. Entities and Properties are given unique identifiers, QIDs and PIDs, respectively. For example, the fact that Joe Biden is the president of the US can be represented as a triple (Q6279, P39, Q11696), where P39 is the PID for property {\em position held}, Q6279 and Q11696 are QIDs for Joe Biden and the president of the United States, respectively. 

Not only is Wikidata large, but unlike relational databases and Freebase, it has no predefined domains or types. It has a set of pre-defined properties; about 3,000 of them are useful for question answering, whereas the rest are used to link data in Wikidata with external library catalogs and database IDs. 


These properties are inconsistent: the same type of information may be represented with different properties. 
%The same question may map to different target properties depending on not just the type of the entities of interest, but also unmentioned attributes of the entity, or even which of the properties have been populated with values. 
As explained below, a seq2seq semantic parser that directly translates a sentence to its logical form would need to memorize the knowledge base to predict the logical form properly and the parser would need to be retrained to accommodate updates in the knowledge base. 

Our philosophy is that the same query on different entities in the same domain should have the same logical form regardless of the properties the entities possess. Thus, our approach is to create an abstract notation that covers the knowledge in terms of domains and properties.  

%Our approach is to create a high-level domain and type hierarchy for property-based graphs so they can have the benefits of types: Entities in the same domain often share the same properties, and hence are asked the same kind of questions. The same question on two different entities will map to a similar logical form. In the following, we describe how we handle domains and properties in Wikidata. 


%The previous method used in synthesizing data for Wikidata is based on choosing a random fact in the knowledge base and generating a corresponding natural language question on that fact. This approach does not provide a good coverage of the questions that can be asked, as discussed in Section~\ref{sec:property-hierarchy}. To better and more efficiently cover possible questions on the knowledge base, we adopt a schema-based approach which (1) synthesizes questions for each domain, their properties, and combinations thereof, and (2) augments the questions with sample entities. In the following, we describe how we apply such an approach to the property-based Wikidata. 

\subsection{Abstract Open Knowledge Domains}
Even though Wikidata is property-based, all named entities have one or more {\em instance of} properties to some domain entity; domain entities are organized into a hierarchy with the {\em subclass of} property. 

Wikidata has over 150K domains and most of them are too subtle to distinguish in natural language and too sparsely used to make meaningful queries. For example, Washington DC is an {\em instance of} ``big city'', ``capital city'', ``human settlement'', and ``planned community'' among others. ``Big city'' and ``capital city'' can be better represented using property {\em population} and {\em capital of} property, while ``human settlement'' and ``planned community'' are just too rare to use in natural language and difficult to distinguish from ``city''.

%\TODO{Schema.org is also hierarchical? You didn't define first-class or top-level} - yes, it is hierarchical
In contrast, Schema.org is a curated ontology for open domain knowledge to facilitate semantic search of web data. Most of the more important Wikidata domains have been mapped to the Schema.org classes via the \property{equivalent class} property. 
%We found our sampling strategy produced a sufficiently large schema to cover questions in \DATASET. 
\begin{comment}
We refer to such domains as {\em abstract}. 
{\em Only} abstract domains are used in our predicted queries. \TODO{PUT IN AN EXAMPLE} For example, Hefei is a ... The query "show me all the cities that is referred to as SELECT ?x WHERE  { ?x    wdt:P31.  /  wdt:P279*   wd:Q515 . } where ....  All the subdomains are implicit ... 
A million-city domain is represented as a city with population of at least 1 million people. 
\end{comment}
%We thus use the Schema.org topology to identify the first-class domains; all domains of Wikidata are either equivalent or a subdomain of these domains, hence all domains in Wikidata are represented. 
%We thus identify the {\em first-class domains} in Wikidata as the domains with an equivalent class in Schema.org topology; all other domains are subdomains of first-class domains, and inherit their properties. 
%An entity is categorized into one of the first-class domains if it is an {\em instance of} the domain, or a subdomain of the domain.  
We refer to such domains as {\em abstract domains}.
We collect the properties of each abstract domain by sampling Wikidata. We first extract the popular entities for each domain based on the number of sitelinks\footnote{\url{https://www.wikidata.org/wiki/Help:Sitelinks}} (number of links for an entity to other Wikimedia pages). We include properties only if they are used by at least two of the top 100 most popular entities in each domain. Note that the sampling size and focus can easily be adjusted. 
%\TODO{Should we move this to implementation?} 
%Silei: agree
%Domains with fewer than 100 entities are dropped.
%In total, we included 180 abstract domains with an average of 28.6 properties per domain. 
%\TODO{Describe how we went from 802 to 180 domains.} - 362 domains with "equivalent class" in schema.org, and 180 of them have at least 100 entities. 
%We found our sampling strategy produced a sufficiently large schema to cover questions in \DATASET. 

%\TODO{Describe the path notation for these superdomains}
\begin{comment}
\TODO{Explain this - from the slides}
    Missing domains in Schema.org
    Identify based on mention in the question
    Considered as a subdomain of one of the key domains
\TODO{Give examples}
Silei: this is confusing to explain here because in SPARQL, everything is represented using "instance of", first-class or not. 
The only difference would be in how we handle entity linking if we factor out thingtalk. I will add an example in that section. 
\end{comment}


\subsection{Abstract Properties}
\label{sec:property-hierarchy}

The target property of a question can depend on the type of the entities of interest, unmentioned attributes of the entity, and which of the properties have been populated with values.
For instance, consider the common question ``where is $x$ located''.  The most likely target property is {\em located in the administrative territorial entity} (P131). However, if $x$ is an organization, then the target property is {\em headquarters location} (P159). If $x$ is a person, then their location can be answered with one of the {\em residence} (P551), {\em work location} (P937), and {\em country of citizenship} (P27) properties, sorted in order of preference.  For the question ``who plays role $x$ in movie $y$'', the target property is {\em voice actor} if the character role is a CGI character, and {\em cast member} otherwise. Such information may not even be available in Wikidata. 

%The principle for our approach is that neural networks should not need to learn these nuances and idiosyncrasies for every entity in the enormous knowledge base. The neural network should simply predict the semantics of the question, and let the predicted logical form be resolved separately for the specific instances depending on what is available in the knowledge base. 

Following our principle of representing the semantics of the query without regards of its implementation, we introduce the concept of an {\em abstract property} to group together concrete properties with similar semantics.  There are two flavors of abstract properties: 
\begin{itemize}
\item
The \textsc{any} abstract property uses the first populated property from an ordered list of sub-properties. For example, {\em location} is an abstract property for {\em located in the administrative territorial entity}, {\em headquarters location}, {\em residence}, {\em state}, {\em country}, {\em continent}, among many others. If a value is available for property {\em located in the administrative territorial entity}, then it will be returned; otherwise, it will check if the value for {\em headquarters location} is available. It will keep searching until it reaches the end of the list. This can be computed with the \textsc{coalesce} operator in SPARQL. 
\item
The \textsc{all} abstract property returns the values for all properties in its list. For example, {\em partner} will return values for both {\em unmarried partner} and {\em spouse}. This can be computed with the \textsc{union} operator in SPARQL.
%\TODO{Is this an OR in Sparql?}
\end{itemize}

Generic questions such as ``where is $x$ located'' will be annotated with the abstract property, {\em location}. After the parse, the predicted abstract property is expanded into the SPARQL code accordingly and executed. 
However, questions asking explicitly for a particular concrete property should parse directly into queries for that property. For example, ``what country is $x$ a citizen of'' is mapped to the property {\em country of citizenship} and not the {\em location} abstract property. It returns null if the \property{country of citizenship} property is not available for $x$. 

We highly recommend that the Wikidata community adopt these abstract properties. Today, only a set of approved Wikidata users are allowed to create properties, and they would be the logical group to curate the abstraction for the 3,000 properties used to answer questions in natural language. 

\iffalse

As discussed above, Wikidata is sparse and different properties could be used to represent the same information for different entities. 
Existing KBQA approaches solve this by traversing the neighborhood of entities and checking what properties are available for those entities, which requires a more complicated training algorithm and longer execution time. More importantly, these approaches are very likely to get an incomplete list of answers for many questions. For example, if we ask for people (e.g. Academy Awards winners) who live in the United States, these approaches either needs to check what property are available for every candidate which would be very inefficient, or it will use {\em residence} property and lose a lot of entities which do not have such property available.  


These issues have led to the common approach of subgraph extraction, which cannot benefit from transfer learning that is afforded by typed schemas. 

This cannot generate any questions that seeks an entity given the properties, such as ``which is the tallest building''. Its distribution is skewed towards the popularity of entities and properties, which does not provide the best coverage.  
\fi

\begin{comment}

How do we synthesize -
> sample all the domains
> generate all possible operations over most of the properties of a given domain
   - sampling of properties
   - super properties 
> combine queries across domains 
> augment with proper values for each property

(why it's harder than relational db)

How do I sample? 
Organize by domains
"prototypes" in type theory - 

Many properties. 

Entities are organized in "domains"
instance-of and subclass: super properties because they all have them. 
entities that have subclasses or targets pf instance-of are domains. 
Domains are hierarchies.

150K domains. 
Distinction is not meaningful.
Have been mapped to the x schema.org
we are using schema.org domains. 
\end{comment}





==> problem.tex <==
\section{Challenges of Semantic Parsing for Large Knowledge Bases}
\label{sec:challenges}

There are over 100 million entities and 10,000 properties in Wikidata. The scale, sparsity, and crowd-sourced nature of Wikidata bring unique challenges to answering questions over Wikidata. In this section, we discuss these challenges in detail. 
%To uniquely identify them, the SPARQL queries for Wikidata uses unique entity IDs (QID) and property ID (PID) to represent entities and properties, respectively. 
%mostly triples where (subject, property, object), where the subject and object are represented by unique entity IDs (QID) and the property is represented as PID. 

\subsection{Named Entities Disambiguation} 
For a closed-domain database, entities are normally unambiguous and can be identified easily by using a soft search. In large knowledge bases like Wikidata, there are lots of entities that share similar or the same names, making it inaccurate to rely on search without context especially since the mentions of each entity often do not exactly match its full name in the knowledge base. In SPARQL, all entities are represented using QIDs, which are unique identifiers for entities. With over 100 million entities in Wikidata, we do not expect the semantic parser to memorize all the different QIDs. 

Previous proposed techniques evaluated with dedicated entity-linking benchmarks did not perform well on \DATASET. 
First, since the dataset is collected from real-world questions without prompting the users on what entities to use, users tend to refer to their entities of interest without using their full names. Secondly, the questions are generally short with very limited context, making it harder to disambiguate entities with entities having similar names. Last but not least, many QIDs in Wikidata are used to represent terms not generally known as ``named entities''. For example, ``domain'' entities are often ignored by entity linkers, as in ``What is the biggest country in Europe by population?'', both ``country'' (Q6256) and ``Europe'' (Q46) are required to construct the correct SPARQL, but entity linkers only provide ``Europe'' and ignores ``country''. 

\TODO{You need a name for the multi-stage parsing strategy.  I can claim you are too because you are using an NED too.}
Note that, the current state-of-the-art approaches use a multi-stage parsing strategy and rely on subgraph extraction based on the entity-linking results at the first stage. Any mistakes made are impossible to recover from. 
\TODO{Please collect these to include in a comparison at the end of performance analysis.}

% todo: discuss this in training strategy
%With suboptimial entity linking accuracy, it's important for the semantic parser to recover from entity linking failures. 

\subsection{Untyped Domains}
Unlike relational databases and Freebase, Wikidata has no predefined domains or types, but only properties. Moreover, the properties are used inconsistently, and the same type of information may be represented with different properties. This makes it hard for semantic parsers to predict the logical form. 

The same question may map to different target properties depending on the entity type, unmentioned attributes of the entity, or simply the availability of information.  
Consider a common question such as ``where is $x$ located'', the most likely target property used is {\em located in the administrative territorial entity} (P131). However, If $x$ is an organization, then the target property is {\em headquarters location} (P159). If $x$ is a person, then their location depends on the availability of information any of the {\em residence} (P551), {\em work location} (P937), and {\em country of citizenship} (P27) properties, sorted in order of preference.  For the question ``who plays role $x$ in movie $y$'', the target property is {\em voice actor} if the character role is a CGI character, and {\em cast member} otherwise. Such information may not even be available in Wikidata. 

These issues have led to the common approach of subgraph extraction, which cannot easily transfer learning that is afforded by typed schemas. 

% discuss how to solve it later
%This makes it difficult for the neural network to predict the logical form without looking at the knowledge \TODO{don't understand} one entity at a time. 

==> schema.tex <==
\section{A Reduced-Resolution Schema for Efficient Synthesis}
Wikidata is noisy and sparse, making it challenging for neural model to process. In this section, we introduce how we can reduce the resolution of Wikidata by giving it a Schema.org-based relational schema.

\subsection{Schema.org Schema over Wikidata}
Different from Freebase, there is no domain schema enforced to constrain how entities and properties can be connected in Wikidata. This makes Wikidata much more flexible and easier to maintain \citep{vrandecic_2013}. 
However, most triples won't make sense to ask in reality. For example, it does not make sense to ask ``who is the spouse of the United States'' since ``spouse'' property should not be used on a country. To efficiently synthesize high-quality data that are meaningful to ask, we adopt a relational database design: we separate entities into domains based on ``instance of'' and ``subclass of'' property, and each domain has a fixed schema listing all meaningful properties for the domain. 

Due to the nature of its flexible design, there are over 150 thousand domains, and most of them are too subtle to distinguish in natural language and too sparsely used to make meaningful queries. For example, Washington DC is an ``instance of'' big city, capital city, human settlement, and planned community among others. Big city and capital city can be better represented using property ``population'' and ``capital of'' property, while human settlement and planned community are just too rare to use in natural language and difficult to distinguish from city.
To reduce the resolution of Wikidata, we leverage carefully crafted domains from Schema.org \citep{guha2016schema} to extract first-class domains, and the rest of the domains are considered subdomains of first-class domains which will be represented by using a filter on the ``instance of'' property. 

Properties for each domain are decided by sampling properties of popular entities: a property is included only if at least two entities among the top 100 sampled entities have it.
Popular entities are extracted based on the number of sitelinks\footnote{\url{https://www.wikidata.org/wiki/Help:Sitelinks}} (number of links for an entity to other Wikimedia pages)
In total, we included 180 top-level domains with an average of 28.6 properties per domain.

\begin{comment}
\subsection{Hierarchical type system}
Since we want to teach the model the schema with synthetic data, it's important to teach the model what properties can be used together. 

For each property, we decide their type based on the sampled 100 example values.
The type for each property is an abstract parent entity type, where all possible domains of its value entities are subtypes. 
Parameter passing is only allowed between properties that share at least one subtypes.

By enforcing such a hierarchical type system, we can synthesize high-quality multi-hop questions based on what domain the value of a property could belongs to. 
This also allows us to understand what entities can be used as values given a property, so that we can efficiently augment synthetic data with different values.
\end{comment}


\subsection{Meta property}
Wikidata is sparse and different properties could be used to express the same semantic for different entities. 
For example, when asking ``where is X located'', the most common property to be used is {\em located in the administrative territorial entity} (P131). However we probably want to use property {\em residence} (P551) if ``X'' is a person and {\em headquarters location} (P159) if ``X'' is a company or organization. And even for the entities within the same domain, different properties may be available for different entities. For example, for people, if {\em residence} property is not available, {\em work location} (P937) is likely to be the next closest answer to the question; and if {\em work location} is also not available, we can use {\em state} or {\em country of citizenship} (P27) as a fallback which has much better availability among human entities. 

Existing KBQA approaches solve this question by traversing the neighborhood of entities and check what properties are available, which requires more complicated training algorithm and execution time. More importantly, these approach is very likely to get an incomplete list of answers for lots of questions. For example, if we ask for people (e.g, Academy Awards winners) who live in the United States, these approaches either needs to check what property are available for every candidates which would be very inefficient, or it will use {\em residence} property and lose a lot of entities which do not have such property available.  

The principle for our approach is that neural networks should not need to learn these nuances and idiosyncrasies for every entity in the enormous knowledge base. Similar to human, the model should be able to understand the general semantic meaning of the questions, and resolve exactly what property to be used afterwards. To achieve this goal, we introduce the concept of {\em meta property}. It represents a group of properties that share similar semantics, to reduce the resolution of Wikidata schema. 
We introduced two types of meta properties: \textsc{any} meta property and \textsc{all} meta property:

\textsc{any} meta property will use the first available property for the entity. For example, {\em location} is a meta property for {\em located in the administrative territorial entity}, {\em headquarters location}, {\em residence}, {\em state}, {\em country}, {\em continent}, among many others. If a value is available for property {\em located in the administrative territorial entity}, then it will be returned; otherwise, it will check if the value for {\em headquarters location} is available. It will keep searching until it reaches the end of the list.
This can be achieved by using the ``COALESCE'' keyword in SPARQL. 

\textsc{all} meta property, on the other hand, will return the values for all properties in its list. For example, {\em partner} will return values for both {\em unmarried partner} and {\em spouse}. 

Note that if a question is explicitly asking for a particular property, meta property won't be applied. E.g., for the question ``what country is X a citizen of'', we will directly go with property ``country of citizenship'' instead of the generic ``location'' meta property. And if no value is available for such question, the model should predict null, i.e., information not available. 

The meta properties are created manually based on the dev set in \DATASET. 
Compared to the size of entities in large knowledge bases, the number of properties are small. 
We think this is an affordable solution to make the Wikidata much easier to be accessed in natural language. 

\subsection{\TT query language}
We extended ThingTalk introduced by \citet{schema2qa} to support common graph queries and meta properties, namely \TT. 
For example, the question ``who is the president of the United States'' can be represented by the following \TT query:
\begin{align}
\small
\textit{@human}\text{()} \texttt{ filter } \texttt{contains} \text{( } \textit{position\_held}, \text{"Q11696")} \nonumber    
\end{align}
where $\textit{@human}$ is the domain of the subject, and ``Q11696'' is the item identifier for the president of the United States.

Different from other intermediate representations used in previous KBQA work, \TT uses a relational database design with a strong type system and similar expressiveness as SPARQL. It also provides an extra abstraction layer over knowledge base properties to remove artificial distinctions across entities. 
Table~\ref{table:tt-syntax} shows the query types and predicate types supported by \TT. A conversion tool is built to convert SPARQL to \TT and from \TT to SPARQL.

\begin{table*}
\small

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{llll}
\toprule
Query type & Syntax & Example  \\
\midrule
Selection           & $q$ \texttt{filter} $\rho$ & \textit{@city}() \texttt{filter} \textit{population} \texttt{>=} 10000  \\
Projection          & [$p^+$] \texttt{of} $q$    & [ \textit{population} ] \texttt{of} \textit{@city}() \\
                    & [$p$ \texttt{filter} $\rho$] \texttt{of} $q$   & [ \textit{population} \texttt{filter} \textit{point\_in\_time} \texttt{==} 2000 ] \texttt{of} \textit{@city}() \\
Verification        & [$\rho$] \texttt{of} $q$   & [ \textit{population} \texttt{>=} 10000 ] \texttt{of} \textit{@city}() \\ 
Sort                & \texttt{sort} ( $p$ \texttt{asc|desc} \texttt{of} $q$ ) & \texttt{sort} (  \textit{population} \texttt{desc} \texttt{of} \textit{@city}() ) \\
Indexing            & $q$[$i$] & \texttt{sort} (  \textit{population} \texttt{desc} \texttt{of} \textit{@city}() )[1]\\
Slicing             & $q$[$i$, $j$] & \texttt{sort} (  \textit{population} \texttt{desc} \texttt{of} \textit{@city}() )[1, 3]\\
Aggregation         & \texttt{count}($q$)  & \texttt{count}(\textit{@city}())\\
                    & \textit{agg}($p$ \texttt{of} $q$) & \texttt{max} (\textit{population} \texttt{of} \textit{@city}())\\
Group By            & \textit{agg}($p_1$ \texttt{of} $q$) \texttt{by} $p_2$ & \texttt{max} (\textit{population} \texttt{of} \textit{@city}()) \textit{by} \textit{country}\\
Join                & $q_1$ \texttt{join} $q_2$ \texttt{on} $p_1$ \textit{op} $p_2$ & \textit{@city}() \texttt{join} \textit{@city}() \texttt{on} \texttt{contains}(\textit{twin\_admin\_body}, \textit{id}) \\
\bottomrule
\end{tabular}
\caption{Supported types of a query $q$ in \TT. $p$ denotes a property in Wikidata, $\rho$ denotes a predicate as shown in Table~\ref{table:tt-predicate}}.
\vspace{10pt}
\label{table:tt-query}
\end{subtable}


\begin{subtable}{\linewidth}
\centering
\begin{tabular}{lll}
\toprule
Predicate type & Syntax & Example  \\
\midrule
Property                & \textit{p} \textit{op} $v$ & \textit{population} \texttt{>=} 10000 \\
Property path           & $p_1^{+|*|?}$/$p_2^{+|*|?}$  & \textit{country} / \textit{population} \texttt{>=} 10000\\
Subquery                & \textit{p} \textit{op} \texttt{any}(\textit{q})  & \textit{population} \texttt{>=} \texttt{any}( [\textit{population}] \texttt{of} \textit{@country}() )\\
Qualifier               & ($p_1$ \texttt{filter} $p_2$ $\textit{op}_2$ $v_2$) $\textit{op}_1$ $v_1$ & ( \textit{population} \texttt{filter}
\textit{point\_in\_time} <= 2000.01.01 ) \texttt{>=} 10000 \\
Aggregation             & \textit{agg}($p$) \textit{op} $v$ & \texttt{count}( \textit{twin\_admin\_body} ) \texttt{>=} 10\\
\texttt{AND}            & $\rho_1$ \texttt{\&\&} $\rho_2$ & \textit{population} \texttt{>=} 10000 \texttt{\&\&} \textit{population} \texttt{<=} 20000 \\
\texttt{OR}             & $\rho_1$ || $\rho_2$ & \textit{population} \texttt{>=} 10000 || \texttt{count}( \textit{twin\_admin\_body} ) \texttt{>=} 10 \\ 
\texttt{NOT}            & $!\rho$              & !( \textit{capital\_of} == NULL )\\

\bottomrule
\end{tabular}
\caption{Supported types of predicate $\rho$ in \TT: $q$, $p$, $v$ denote a query, a property, and a value, respectively. Property path is similar to SPARQL property path \cite{sparql_property_path} to simplify the representation of common joins/subqueries. It supports sequence path, zero or more path, one or more path, and zero or one path.} 
\label{table:tt-predicate}
\end{subtable}


\caption{\TT Syntax}
\label{table:tt-syntax}
\end{table*}

==> solution.tex <==
\section{Taming Large Knowledge Graphs}
% Challenges for semantic parsing for large knowledge graph

Our solution is to train an NED for Wikidata, and also train the semantic parser to recover from unmentioned entities. 

Our solution is to introduce a type hierarchy to organized the relatively small number of properties, akin to how domains have a type hierarchy. 

%To overcome the unique challenges of semantic parsing over large knowledge bases, we propose a synthesis-based training paradigm where high-quality synthetic data is used to provide coverage over domains and properties in Wikidata. 

\subsection{Representation}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/overview.pdf}
    \caption{The input and output of the semantic parser.}
    \label{fig:overview}
\end{figure}

As discussed in Section~\ref{sec:challenges}, named entities are difficult to distinguish with just names. Thus 
the logical form of each query needs to use QIDs to represent the entities mentioned in the question. 
On the other hand, since properties can be identified by name, we can keep the name of the property in the logical form to make it easier to be trained 
by language models.

Following this principle, we choose ThingTalk introduced by \citet{schema2qa} for database query as our logical form, 
with extensions to better support graph queries. 
For example, the question ``who is the president of the United States'' can be represented by the following \TT query:
\begin{align}
\small
\text{[}\textit{head\_of\_state}\text{]} \texttt{ of } \text{@entity}\text{()} \texttt{ filter } \textit{id} == \text{"Q30"} \nonumber    
\end{align}
where {\em head\_of\_state} represents the {\em head of state} property by name, and ``Q30'' is the item identifier for the United States.

During training and evaluation, an entity linker is used to first identify the named entities mentioned in the question. 
For each named entity identified, the span of its mention in the question and its domain are appended to the question along with its QID.
The semantic parser takes the question appended with entity information as its input, and outputs \TT directly, as shown in Figure~\ref{fig:overview}.

In case the entity linker failed to provide the QID of the correct entities, the entities are represented with their corresponding spans in the utterance in \TT for all data. 
During inference time, we look up the QID for each entity whose QID is missing after the model predicts the \TT representation. 
This allows the model to potentially recover from entity-linking failures to get the correct answers. 

A conversion tool is built to convert SPARQL to \TT and from \TT to SPARQL.
All data in \DATASET is converted into \TT for training, and at inference time, once \TT is predicted, it's converted back into SPARQL to retrieve the answers from Wikidata. 


\subsection{Coverage by Synthesis}
Training data synthesis has been widely used to provide training data for semantic parsing tasks. 
The synthesis approach can be divided into two categories: fact-based synthesis and schema-based synthesis. 

The fact-based synthesis starts with a random fact in the knowledge base and then generates the corresponding natural language question to ask about a part of the fact. 
It has been widely used for generating KBQA examples but it often has suboptimal coverage over the whole knowledge base,
as it does not have the concept of domains and tends to emphasize popular entities and properties instead of long tails. 

The schema-based synthesis, on the other hand, generates questions based on domains and their schema which defines what properties are available for a given domain. It evenly generates questions for all possible properties and their combinations, and the generated questions can then be augmented with proper values for each domain. 
We adopt this synthesis approach as it provides better coverage over the underlying knowledge base. 

However, different from Freebase, there is no domain schema enforced to constrain how entities and properties can be connected in Wikidata.
In the following, we introduce {\em meta domains} and {\em meta properties} to organize entities and properties. 

\subsubsection{Meta domains}
Entities in Wikidata can be loosely categorized into domains based on the {\em instance of} property. However, there will be over 150 thousand domains and most of them are too subtle to distinguish in natural language and too sparsely used to make meaningful queries. For example, Washington DC is an {\em instance of} ``big city'', ``capital city'', ``human settlement'', and ``planned community'' among others. ``Big city'' and ``capital city'' can be better represented using property {\em population} and {\em capital of} property, while ``human settlement'' and {\em planned community} are just too rare to use in natural language and difficult to distinguish from ``city''.

To reduce the resolution of Wikidata, we choose domains that have equivalent Schema.org classes as our first-class domains. 
Schema.org classes are carefully crafted for the schema of web data, and widely adopted by web pages for better semantic search. It provides a more refined set of domains which includes most of the common ones in real-world questions. Other domains in Wikidata can be represented as subdomains of first-class domains if specifically asked. 

Properties for each domain are decided by sampling properties of popular entities: a property is included only if at least two entities among the top 100 sampled entities have it.
Popular entities are extracted based on the number of sitelinks\footnote{\url{https://www.wikidata.org/wiki/Help:Sitelinks}} (number of links for an entity to other Wikimedia pages)
In total, we included 180 top-level domains with an average of 28.6 properties per domain. We found the sampling strategy we used produced a sufficiently large schema to cover questions \DATASET. However, the sampling size can be easily increased if better coverage is desired. 


\subsubsection{Meta properties}
As discussed in Section~\ref{sec:challenges}, Wikidata is sparse and different properties could be used to express the same semantics for different entities. 
Existing KBQA approaches solve this by traversing the neighborhood of entities and checking what properties are available, which requires a more complicated training algorithm and longer execution time. More importantly, these approaches are very likely to get an incomplete list of answers for lots of questions. For example, if we ask for people (e.g, Academy Awards winners) who live in the United States, these approaches either needs to check what property are available for every candidate which would be very inefficient, or it will use {\em residence} property and lose a lot of entities which do not have such property available.  

The principle for our approach is that neural networks should not need to learn these nuances and idiosyncrasies for every entity in the enormous knowledge base. Similar to humans, the model should be able to understand the general semantic meaning of the questions and only resolve exactly what property to be used after the logical form is predicted. To achieve this goal, we introduce the concept of {\em meta property}. It represents a group of properties that share similar semantics, to reduce the resolution of Wikidata schema. 
We introduced two types of meta properties: \textsc{any} meta property and \textsc{all} meta property:

\textsc{any} meta property will use the first available property for the entity. For example, {\em location} is a meta property for {\em located in the administrative territorial entity}, {\em headquarters location}, {\em residence}, {\em state}, {\em country}, {\em continent}, among many others. If a value is available for property {\em located in the administrative territorial entity}, then it will be returned; otherwise, it will check if the value for {\em headquarters location} is available. It will keep searching until it reaches the end of the list.
This can be achieved by using the ``COALESCE'' keyword in SPARQL. 

\textsc{all} meta property, on the other hand, will return the values for all properties in its list. For example, {\em partner} will return values for both {\em unmarried partner} and {\em spouse}. 

Note that if a question is explicitly asking for a particular property, meta property won't be applied. E.g., for the question ``what country is X a citizen of'', we will directly go with property ``country of citizenship'' instead of the generic ``location'' meta property. And if no value is available for such question, the model should predict null, i.e., information not available. 

The meta properties are created manually based on the dev set in \DATASET. 
Compared to the size of entities in large knowledge bases, the number of properties is small. 
We think this is an affordable solution to make Wikidata much easier to be accessed in natural language.

\begin{comment}
How do we synthesize -
> sample all the domains
> generate all possible operations over most of the properties of a given domain
   - sampling of properties
   - meta properties 
> combine queries across domains 
> augment with proper values for each property

(why it's harder than relational db)

How do I sample? 
Organize by domains
"prototypes" in type theory - 

Many properties. 

Entities are organized in "domains"
instance-of and subclass: super properties because they all have them. 
entities that have subclasses or targets pf instance-of are domains. 
Domains are hierarchies.

150K domains. 
Distinction is not meaningful.
Have been mapped to the x schema.org
we are using schema.org domains. 
\end{comment}

